Blockchain scaling and liquidity concentration on decentralized exchanges

Liquidity providers (LPs) on decentralized exchanges (DEXs) can protect themselves from adverse selection risk by updating their positions more frequently. However, repositioning is costly, because LPs have to pay gas fees for each update. We analyze the causal relation between repositioning and liquidity concentration around the market price, using the entry of blockchain scaling solutions, Arbitrum and Polygon, as our instruments. Lower gas fees on scaling solutions allow LPs to update more frequently than on Ethereum. Our results demonstrate that higher repositioning intensity and precision lead to greater liquidity concentration, which benefits small trades by reducing their slippage.

==> Files/estimation_arbdrop_usdc_eth_005_pres.tex <==
\begin{tabularx}{\textwidth}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{13}{l}{ \textbf{Panel A: USDC/(W)ETH 0.05\%}} \\  \hline 
 & \multicolumn{6}{c}{Before Airdrop} & \multicolumn{6}{c}{After Airdrop} \\  
 & Int & & Conc & & Conc & & Int & & Conc & & Conc &    \\ 
 &  & & $ 2\%$ & & $ 2\%$ & & &  & $ 2\%$ & & $ 2\%$ &    \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$Arbitrum$          &        0.22&         ***&            &            &            &            &        0.35&         ***&            &            &            &            \\
                    &     (31.23)&            &            &            &            &            &     (17.93)&            &            &            &            &            \\
$Intensity$         &            &            &        0.04&         ***&            &            &            &            &        0.29&         ***&            &            \\
                    &            &            &     (29.71)&            &            &            &            &            &     (35.37)&            &            &            \\
$Precision$         &            &            &            &            &        0.05&         ***&            &            &            &            &        0.68&         ***\\
                    &            &            &            &            &     (13.90)&            &            &            &            &            &      (7.11)&            \\
\midrule
$ Observations$     &      87,698&            &      87,698&            &      33,849&            &      27,119&            &      27,119&            &      14,138&            \\
$ HourFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
$ DateFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
\bottomrule
\end{tabularx}


==> Files/estimation_int_usdc_eth_005_pres.tex <==
\begin{tabularx}{\textwidth}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel A: USDC/(W)ETH 0.05\%}} \\  \hline 
 & \multicolumn{4}{c}{Arbitrum} & \multicolumn{4}{c}{Polygon} & \multicolumn{4}{c}{BlockScaling}  \\ 
 & Int & & Conc & & Int & & Conc & & Int & & Conc &    \\ 
 &  & & $ 2\%$ & & $ & & $ 2\%$ & &  & & $ 2\%$ &    \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$Arbitrum$          &        0.24&         ***&            &            &            &            &            &            &            &            &            &            \\
                    &     (35.55)&            &            &            &            &            &            &            &            &            &            &            \\
$Polygon$           &            &            &            &            &        0.20&         ***&            &            &            &            &            &            \\
                    &            &            &            &            &     (33.60)&            &            &            &            &            &            &            \\
$BlockScaling$      &            &            &            &            &            &            &            &            &        0.21&         ***&            &            \\
                    &            &            &            &            &            &            &            &            &     (43.78)&            &            &            \\
$Intensity$         &            &            &        0.09&         ***&            &            &        0.11&         ***&            &            &        0.11&         ***\\
                    &            &            &     (59.67)&            &            &            &     (66.04)&            &            &            &     (69.65)&            \\
\midrule
$ Observations$     &     114,817&            &     114,817&            &     148,416&            &     148,416&            &     221,268&            &     221,268&            \\
$ HourFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
$ DateFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
\bottomrule
\end{tabularx}


==> Files/estimation_int_usdc_eth_005_r1.tex <==
\begin{tabularx}{\textwidth}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{13}{l}{ \textbf{Panel A: ETH/USDC 0.05\%}} \\  \hline 
 & \multicolumn{4}{c}{Arbitrum} & \multicolumn{4}{c}{Polygon} & \multicolumn{4}{c}{BlockScaling}  \\ 
 & Int & & Conc & & Int & & Conc & & Int & & Conc &    \\ 
 &  & & $ 2\%$ & &  & & $ 2\%$ & &  & & $ 2\%$ &    \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$Arbitrum$          &        0.17&         ***&            &            &            &            &            &            &            &            &            &            \\
                    &     (27.45)&            &            &            &            &            &            &            &            &            &            &            \\
$Polygon$           &            &            &            &            &        0.13&         ***&            &            &            &            &            &            \\
                    &            &            &            &            &     (21.14)&            &            &            &            &            &            &            \\
$BlockScaling$      &            &            &            &            &            &            &            &            &        0.14&         ***&            &            \\
                    &            &            &            &            &            &            &            &            &     (29.46)&            &            &            \\
$Intensity$         &            &            &        0.13&         ***&            &            &        0.16&         ***&            &            &        0.16&         ***\\
                    &            &            &     (60.44)&            &            &            &     (66.52)&            &            &            &     (71.87)&            \\
$Volume$            &       -0.01&         ***&        0.01&         ***&       -0.02&         ***&        0.01&         ***&       -0.00&            &        0.01&         ***\\
                    &     (-3.53)&            &     (60.41)&            &     (-4.33)&            &     (68.53)&            &     (-1.28)&            &     (69.84)&            \\
$Volatility$        &       -0.25&            &       -1.55&         ***&        0.58&            &       -1.61&         ***&       -0.70&          **&       -1.44&         ***\\
                    &     (-0.71)&            &    (-42.82)&            &      (1.29)&            &    (-50.40)&            &     (-2.00)&            &    (-51.67)&            \\
$|Return|$          &       19.97&         ***&       -3.30&         ***&       14.88&         ***&       -2.91&         ***&       19.45&         ***&       -3.71&         ***\\
                    &     (15.82)&            &    (-27.64)&            &     (15.37)&            &    (-30.00)&            &     (18.06)&            &    (-38.80)&            \\
\midrule
$ Observations$     &     114,816&            &     114,816&            &     148,415&            &     148,415&            &     221,267&            &     221,267&            \\
$ HourFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
$ DateFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
\bottomrule
\end{tabularx}


==> Files/estimation_int_usdc_eth_030_r1.tex <==
\begin{tabularx}{\textwidth}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{13}{l}{ \textbf{Panel B: ETH/USDC 0.3\%}} \\  \hline 
 & \multicolumn{4}{c}{Arbitrum} & \multicolumn{4}{c}{Polygon} & \multicolumn{4}{c}{BlockScaling}  \\ 
 & Int & & Conc & & Int & & Conc & & Int & & Conc &    \\ 
 &  & & $ 2\%$ & &  & & $ 2\%$ & &  & & $ 2\%$ &    \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$Arbitrum$          &        0.10&         ***&            &            &            &            &            &            &            &            &            &            \\
                    &     (11.07)&            &            &            &            &            &            &            &            &            &            &            \\
$Polygon$           &            &            &            &            &        0.10&         ***&            &            &            &            &            &            \\
                    &            &            &            &            &     (20.09)&            &            &            &            &            &            &            \\
$BlockScaling$      &            &            &            &            &            &            &            &            &        0.09&         ***&            &            \\
                    &            &            &            &            &            &            &            &            &     (18.58)&            &            &            \\
$Intensity$         &            &            &        0.10&         ***&            &            &        0.35&         ***&            &            &        0.21&         ***\\
                    &            &            &     (31.39)&            &            &            &     (39.08)&            &            &            &     (44.66)&            \\
$Volume$            &       -0.17&         ***&        0.07&         ***&       -0.00&            &        0.04&         ***&       -0.02&            &        0.07&         ***\\
                    &     (-5.43)&            &     (53.25)&            &     (-0.26)&            &     (17.45)&            &     (-1.65)&            &     (54.16)&            \\
$Volatility$        &        2.27&         ***&       -1.20&         ***&       -0.24&            &       -0.93&         ***&        0.05&            &       -1.49&         ***\\
                    &      (4.59)&            &    (-45.96)&            &     (-0.73)&            &    (-12.96)&            &      (0.14)&            &    (-35.58)&            \\
$|Return|$          &        6.60&         ***&       -0.86&         ***&       16.46&         ***&       -6.01&         ***&       16.04&         ***&       -3.59&         ***\\
                    &      (8.06)&            &    (-11.76)&            &     (11.81)&            &    (-18.42)&            &     (13.35)&            &    (-21.11)&            \\
\midrule
$ Observations$     &      53,145&            &      53,145&            &      57,472&            &      57,472&            &      81,810&            &      81,810&            \\
$ HourFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
$ DateFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
\bottomrule
\end{tabularx}


==> Files/estimation_prec_usdc_eth_005_pres.tex <==
\begin{tabularx}{11.7cm}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{13}{l}{ \textbf{Panel A: USDC/(W)ETH 0.05\%}} \\  \hline 
 & Gap & & Conc & & Len & & Conc & & Prec & & Conc &    \\ 
 &  & & $ 2\%$ & & & & $ 2\%$ & & & & $ 2\%$ &    \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$BlockScal$      &       -0.01&         ***&            &            &       -0.05&         ***&            &            &        0.12&         ***&            &            \\
                    &     (-9.26)&            &            &            &    (-13.83)&            &            &            &     (11.85)&            &            &            \\
$Gap$               &            &            &       -4.15&         ***&            &            &            &            &            &            &            &            \\
                    &            &            &    (-15.82)&            &            &            &            &            &            &            &            &            \\
$Length$            &            &            &            &            &            &            &       -0.47&         ***&            &            &            &            \\
                    &            &            &            &            &            &            &    (-27.70)&            &            &            &            &            \\
$Prec$         &            &            &            &            &            &            &            &            &            &            &        0.18&         ***\\
                    &            &            &            &            &            &            &            &            &            &            &     (23.28)&            \\
\midrule
$ Obs$     &     102,625&            &     102,625&            &     102,625&            &     102,625&            &     102,625&            &     102,625&            \\
$ HourFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
$ DateFE$ & Yes & & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
\bottomrule
\end{tabularx}


==> Files/estimation_slip_usdc_eth_005_pres.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel B: USDC/(W)ETH 0.05\%}} \\  \hline 
 & \multicolumn{6}{c}{BlockScaling} & \multicolumn{2}{c}{Arbitrum} & \multicolumn{2}{c}{Polygon}  \\ 
 & Total & & Large $>\$1K$ & & Large $>\$5K$ & & Large $>\$1K$ & & Large $>\$1K$ &  \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$BlockScaling$      &        1.41&         ***&       -4.60&         ***&       -4.32&         ***&            &            &            &            \\
                    &      (3.18)&            &     (-9.10)&            &     (-8.65)&            &            &            &            &            \\
$Arbitrum$          &            &            &            &            &            &            &       -6.41&         ***&            &            \\
                    &            &            &            &            &            &            &     (-8.09)&            &            &            \\
$Polygon$           &            &            &            &            &            &            &            &            &       -1.62&         ***\\
                    &            &            &            &            &            &            &            &            &     (-8.73)&            \\
$BlockSc\cdot Large$&            &            &       10.53&         ***&       13.37&         ***&       14.37     & ***   &       6.67 &  		***\\
                    &            &            &     (19.79)&            &     (19.79)&            &      (15.12)&            &      (42.59)    &            \\
$Large$             &            &            &        0.51&         ***&        0.65&         ***&        0.51&         ***&        0.51&         ***\\
                    &            &            &     (37.00)&            &     (37.00)&            &     (37.00)&            &     (37.00)&            \\
$Size$              &        0.19&         ***&            &            &            &            &            &            &            &            \\
                    &     (20.63)&            &            &            &            &            &            &            &            &            \\
\midrule
$ R^2$              &        0.28&            &        0.20&            &        0.24&            &        0.24&            &        0.36&            \\
$ Observations$     &   6,603,702&            &   6,603,702&            &   6,603,702&            &   4,402,468&            &   4,402,468&            \\
$ HourFE$ & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
$ DateFE$ & Yes & & Yes & & Yes & & Yes & & Yes &  \\ 
\bottomrule
\end{tabularx}


==> Files/mintsburns_sumstat_pres.tex <==
\begin{tabular}{cccccc}
\hline
\textbf{Pool}   & \textbf{Mints}    & \textbf{Minted}    & \textbf{Burns}   & \textbf{Burned}    & \textbf{Intensity} \\
\textbf{}       & \textbf{(\#/day)}  & \textbf{(\$M/day)} & \textbf{(\#/day)} & \textbf{(\$M/day)} & \textbf{(\%)}      \\
\hline
ETH/USDC 0.05\% &                                     &                   &                &                    &                    \\
Ethereum        & 81.21                 & 41.19              & 61.54             & 39.90              & 15.89              \\
Arbitrum        & 315.27                 & 11.75              & 237.83           & 11.60              & 40.64              \\
$\Delta Arb-Eth$      & 234.06            & -29.44             & 176.29            & -28.31             & 24.75              \\
         & (137.45)                      & (-29.00)            & (106.40)           & (-28.19)             & (96.64)              \\
Polygon         & 546.64                  & 2.95               & 371.46               & 2.82               & 35.90              \\
$\Delta Pol-Eth$      & 465.43              & -38.24             & 309.92                  & -37.08             & 20.01              \\
        & (246.81)                          & (-40.04)             & (205.67)           & (-39.32)             & (84.01)              \\
\hline
ETH/USDC 0.3\%  &                   &                            &                &                    &                    \\
Ethereum        & 74.18                  & 6.53               & 32.65                  & 5.42               & 7.29            \\
Arbitrum        & 69.92                     & 0.26               & 31.66                  & 0.24               & 17.10            \\
$\Delta Arb-Eth$     & -4.25                   & -6.27              & -0.99                    & -5.18              & 9.81             \\
         & (-4.69)                          & (-26.33)             & (-2.45)                         & (-22.76)             & (36.14)              \\
Polygon         & 72.94                 & 0.30               & 46.88                  & 0.28               & 24.78              \\
$\Delta Pol-Eth$      & -1.24                  & -6.23              & 14.22                 & -5.14              & 17.49              \\
       & (-1.67)                         & (-26.16)             & (30.70)                        & (-22.58)             & (60.39)         
\\\hline
\end{tabular}

==> Files/table1a_pres.tex <==
\begin{tabularx}{10cm}{cccc}
\hline
\textbf{Pool}   & \textbf{Volume 24h (\$M)} & \textbf{TVL (\$M)} & \textbf{Volume/TVL} \\
\hline
ETH/USDC 0.05\% &                           &                    &                     \\
Ethereum        & 513.73                    & 201.19             & 2.55                \\
Arbitrum        & 51.93                     & 18.04              & 2.88                \\
Polygon         & 29.03                     & 10.26              & 2.83                \\
\hline
ETH/USDC 0.3\%  &                           &                    &                     \\
Ethereum        & 57.83                     & 176.59             & 0.33                \\
Arbitrum        & 1.65                      & 4.48               & 0.37                \\
Polygon         & 0.95                      & 1.89               & 0.50 
\\\hline
\end{tabularx}

==> Files/table1b_pres.tex <==
\begin{tabularx}{10cm}{cccccc}
\hline
\textbf{Pool}   & \textbf{Mean (\$K)} & \textbf{SD} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} \\
\hline
ETH/USDC 0.05\% &                     &             &               &               &               \\
Ethereum        & 72.19               & 255.61      & 0.82          & 4.55          & 42.67         \\
Arbitrum        & 4.12                & 10.10       & 0.06          & 0.96          & 4.64          \\
Polygon         & 2.42                & 5.09        & 0.07          & 0.77          & 2.86          \\
\hline
ETH/USDC 0.3\%  &                     &             &               &               &               \\
Ethereum        & 116.19              & 241.02      & 1.31          & 30.00         & 144.65        \\
Arbitrum        & 2.95                & 6.76        & 0.08          & 1.34          & 3.33          \\
Polygon         & 1.74                & 3.37        & 0.38          & 0.88          & 1.83         
\\\hline
\end{tabularx}

==> files_v1/estimation_int_eth_usdt_030.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel C: ETH/USDT 0.3\%}} \\  \hline 
  & $Intensity$ & & \multicolumn{6}{c}{$LiquidityConcentration$} &&      \\ 
 & & & \multicolumn{6}{c}{5min} & \multicolumn{2}{c}{10min}  \\ 
 &  & &  1\% & &  2\% & &  10\% & & 2\% &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$Polygon$           &        0.05&         ***&            &            &            &            &            &            &            &            \\
                    &      (4.82)&            &            &            &            &            &            &            &            &            \\
$Intensity$         &            &            &        0.18&         ***&        0.35&         ***&        0.69&         ***&        0.28&         ***\\
                    &            &            &      (7.02)&            &      (7.02)&            &      (6.89)&            &      (6.04)&            \\
\midrule
$ Observations$             &       7,876&            &       7,876&            &       7,876&            &       7,876&            &       3,943&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                           \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                          \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_int_usdc_eth_005.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel A: ETH/USDC 0.05\%}} \\  \hline 
  & $Intensity$ & & \multicolumn{6}{c}{$LiquidityConcentration$} &&      \\ 
 & & & \multicolumn{6}{c}{5min} & \multicolumn{2}{c}{10min}  \\ 
 &  & &  1\% & &  2\% & &  10\% & & 2\% &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$Polygon$           &        0.18&         ***&            &            &            &            &            &            &            &            \\
                    &     (26.83)&            &            &            &            &            &            &            &            &            \\
$Intensity$         &            &            &        0.05&         ***&        0.10&         ***&        0.30&         ***&        0.10&         ***\\
                    &            &            &     (48.62)&            &     (52.10)&            &     (57.15)&            &     (37.00)&            \\
$Volume$            &        0.01&           *&        0.01&         ***&        0.01&         ***&        0.03&         ***&        0.01&         ***\\
                    &      (1.91)&            &     (59.26)&            &     (58.34)&            &     (54.41)&            &     (39.83)&            \\
$Volatility$             &       -0.58&            &       -0.92&         ***&       -1.63&         ***&       -4.00&         ***&       -1.61&         ***\\
                    &     (-1.15)&            &    (-51.26)&            &    (-49.36)&            &    (-43.40)&            &    (-34.22)&            \\
$|Return|$             &       14.18&         ***&       -1.23&         ***&       -2.12&         ***&       -5.11&         ***&       -1.33&         ***\\
                    &     (12.56)&            &    (-26.61)&            &    (-25.05)&            &    (-20.96)&            &    (-16.99)&            \\
\midrule
$ Observations$             &      88,531&            &      88,532&            &      88,532&            &      88,532&            &      44,646&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                           \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                         \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_int_usdc_eth_005_pres.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel A: ETH/USDC 0.05\%}} \\  \hline 
  & Intensity & & \multicolumn{6}{c}{Liquidity Concentration} &&      \\ 
 & & & \multicolumn{6}{c}{5-minute} & \multicolumn{2}{c}{10-minute}  \\ 
 &  & &  1\% & &  2\% & &  10\% & & 2\% &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$Polygon$           &        0.18&         ***&            &            &            &            &            &            &            &            \\
                    &     (26.83)&            &            &            &            &            &            &            &            &            \\
$Intensity$         &            &            &        0.05&         ***&        0.10&         ***&        0.30&         ***&        0.10&         ***\\
                    &            &            &     (48.62)&            &     (52.10)&            &     (57.15)&            &     (37.00)&            \\

\midrule
$ Obs.$             &      88,531&            &      88,532&            &      88,532&            &      88,532&            &      44,646&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                            \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                          \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_int_usdc_eth_030.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel B: ETH/USDC 0.3\%}} \\  \hline 
  & $Intensity$ & & \multicolumn{6}{c}{$LiquidityConcentration$} &&      \\ 
 & & & \multicolumn{6}{c}{5min} & \multicolumn{2}{c}{10min}  \\ 
 &  & &  1\% & &  2\% & &  10\% & & 2\% &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$Polygon$           &        0.09&         ***&            &            &            &            &            &            &            &            \\
                    &     (20.47)&            &            &            &            &            &            &            &            &            \\
$Intensity$         &            &            &        0.19&         ***&        0.37&         ***&        1.13&         ***&        0.38&         ***\\
                    &            &            &     (25.99)&            &     (26.14)&            &     (26.30)&            &     (18.40)&            \\
\midrule
$ Observations$             &      48,332&            &      48,332&            &      48,332&            &      48,332&            &      24,151&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                            \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                          \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_prec_eth_usdt_030.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel C: ETH/USDT 0.3\%}} \\  \hline 
  & \multicolumn{10}{c}{$LiquidityConcentration$}      \\ 
 & Total & & Total & & Total & & Intraday & & Multiday &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$PositionGap$         &       -3.85&         ***&            &            &            &            &            &            &            &            \\
                    &     (-4.66)&            &            &            &            &            &            &            &            &            \\
$PositionLength$      &            &            &       -0.06&         ***&            &            &            &            &            &            \\
                    &            &            &    (-22.20)&            &            &            &            &            &            &            \\
$PositionConc.$  &            &            &            &            &        0.34&         ***&    -3.03   &            &   0.42     &  ***       \\
                    &            &            &            &            &      (9.07)&            &     (-0.33) &            &    (8.15) &            \\
\midrule
$ Observations$             &       7,876&            &       7,873&            &       7,876&            &       1,052&            &       7,876&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                           \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                          \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_prec_usdc_eth_005.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel A: ETH/USDC 0.05\%}} \\  \hline 
  & \multicolumn{10}{c}{$LiquidityConcentration$}      \\ 
 & Total & & Total & & Total & & Intraday & & Multiday &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$PositionGap$         &       -3.08&         ***&            &            &            &            &            &            &            &            \\
                    &    (-19.54)&            &            &            &            &            &            &            &            &            \\
$PositionLength$      &            &            &       -0.34&         ***&            &            &            &            &            &            \\
                    &            &            &    (-23.00)&            &            &            &            &            &            &            \\
$PositionConc.$  &            &            &            &            &        0.20&         ***&     0.42   &         ***&        0.21& ***        \\
                    &            &            &            &            &     (26.47)&            &     	(7.42)&         &        (29.72)    &     \\
$Volume$            &        0.01&         ***&        0.01&         ***&        0.01&         ***&        0.00&          **&        0.01&         ***\\
                    &     (23.84)&            &     (21.73)&            &     (31.52)&            &      (2.38)&            &     (32.75)&            \\
$Volatility$             &       -1.31&         ***&       -1.21&         ***&       -1.21&         ***&       -0.60&         ***&       -1.33&         ***\\
                    &    (-15.50)&            &    (-18.63)&            &    (-19.68)&            &     (-2.79)&            &    (-24.99)&            \\
$|Return|$             &       -1.92&         ***&       -2.13&         ***&       -1.84&         ***&       -0.76&          **&       -1.38&         ***\\
                    &    (-10.61)&            &    (-14.73)&            &    (-13.70)&            &     (-2.39)&            &    (-11.36)&            \\
\midrule
$ Observations$             &      88,532&            &      88,518&            &      88,532&            &      43,345&            &      88,532&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                            \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                         \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_prec_usdc_eth_005_pres.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel A: ETH/USDC 0.05\%}} \\  \hline 
  & \multicolumn{10}{c}{Liquidity Concentration, 2\%}      \\ 
 & Total & & Total & & Total & & Intraday & & Multi-Day &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$PositionGap$         &       -3.08&         ***&            &            &            &            &            &            &            &            \\
                    &    (-19.54)&            &            &            &            &            &            &            &            &            \\
$PositionLength$      &            &            &       -0.34&         ***&            &            &            &            &            &            \\
                    &            &            &    (-23.00)&            &            &            &            &            &            &            \\
$PositionConcntr$  &            &            &            &            &        0.20&         ***&     0.42   &         ***&        0.21& ***        \\
                    &            &            &            &            &     (26.47)&            &     	(7.42)&         &        (29.72)    &     \\

\midrule
$ Obs.$             &      88,532&            &      88,518&            &      88,532&            &      43,345&            &      88,532&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                           \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                          \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_prec_usdc_eth_030.tex <==
\begin{tabularx}{\textwidth}{l *{5}{R@{ }l}} \\
\toprule
 \multicolumn{11}{l}{ \textbf{Panel B: ETH/USDC 0.3\%}} \\  \hline 
  & \multicolumn{10}{c}{$LiquidityConcentration$}      \\ 
 & Total & & Total & & Total & & Intraday & & Multiday &   \\ 
& (1) & & (2) & & (3) & & (4) & & (5) &  \\ 
\midrule
$PositionGap$         &       -5.71&         ***&            &            &            &            &            &            &            &            \\
                    &    (-11.93)&            &            &            &            &            &            &            &            &            \\
$PositionLength$      &            &            &       -0.08&         ***&            &            &            &            &            &            \\
                    &            &            &    (-74.55)&            &            &            &            &            &            &            \\
$PositionConc.$  &            &            &            &            &        0.34&         ***&     0.36   & ***        &  0.59      &  ***       \\
                    &            &            &            &            &     (32.63)&            &      (8.68)&            &  (22.34)   &            \\
\midrule
$ Observations$             &      48,332&            &      48,323&            &      48,332&            &       8,653&            &      48,332&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                            \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&                         \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_slip_eth_usdt_030.tex <==
\begin{tabularx}{\textwidth}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{13}{l}{ \textbf{Panel C: ETH/USDT 0.3\%}} \\  \hline 
 & \multicolumn{8}{c}{$Slippage$} & \multicolumn{4}{c}{$ExecutionCost$}  \\ 
 & Total & & \$1K cutoff & & \$5K cutoff & & \$10K cutoff& & Total & & \$5K cutoff&  \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$Polygon$           &     6500.29&         ***&       31.13&            &       49.39&            &       77.17&            &     6360.35&         ***&     -347.14&         ***\\
                    &     (37.36)&            &      (0.27)&            &      (0.43)&            &      (0.68)&            &     (35.94)&            &     (-2.99)&            \\
$Polygon\cdot Large$&            &            &     9703.75&         ***&    11611.63&         ***&    14452.02&         ***&            &            &    12073.47&         ***\\
                    &            &            &     (46.99)&            &     (46.99)&            &     (46.99)&            &            &            &     (50.10)&            \\
$Large$             &            &            &       16.82&         ***&       20.07&         ***&       24.85&         ***&            &            &     -442.11&         ***\\
                    &            &            &     (46.55)&            &     (46.56)&            &     (46.56)&            &            &            &    (-14.63)&            \\
$Size$              &       18.86&         ***&            &            &            &            &            &            &       18.68&         ***&            &            \\
                    &     (47.95)&            &            &            &            &            &            &            &     (47.09)&            &            &            \\
\midrule
$ R^2$              &        0.32&            &        0.16&            &        0.20&            &        0.25&            &        0.31&            &        0.19&            \\
$ Observations$             &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_slip_usdc_eth_005.tex <==
\begin{tabularx}{\textwidth}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{13}{l}{ \textbf{Panel A: ETH/USDC 0.05\%}} \\  \hline 
 & \multicolumn{8}{c}{$Slippage$} & \multicolumn{4}{c}{$ExecutionCost$}  \\ 
 & Total & & \$1K cutoff & & \$5K cutoff & & \$10K cutoff& & Total & & \$5K cutoff&  \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$Polygon$           &       18.38&         ***&      -20.12&         ***&      -19.92&         ***&      -19.61&         ***&      -12.97&            &     -307.84&         ***\\
                    &      (6.45)&            &     (-5.72)&            &     (-5.67)&            &     (-5.59)&            &     (-0.69)&            &    (-10.60)&            \\
$Polygon\cdot Large$&            &            &       57.75&         ***&       68.93&         ***&       85.47&         ***&            &            &      530.78&         ***\\
                    &            &            &     (26.72)&            &     (26.69)&            &     (26.65)&            &            &            &     (17.48)&            \\
$Large$             &            &            &        3.99&         ***&        4.76&         ***&        5.90&         ***&            &            &     -457.41&         ***\\
                    &            &            &     (29.75)&            &     (29.75)&            &     (29.75)&            &            &            &    (-15.21)&            \\
$Size$              &        0.12&         ***&            &            &            &            &            &            &       -0.06&         ***&            &            \\
                    &     (26.40)&            &            &            &            &            &            &            &     (-4.81)&            &            &            \\
$Buy$               &       -3.69&         ***&       -3.69&         ***&       -3.69&         ***&       -3.69&         ***&       -3.69&         ***&       -3.69&         ***\\
                    &     (-5.73)&            &     (-5.73)&            &     (-5.73)&            &     (-5.73)&            &     (-5.73)&            &     (-5.73)&            \\
$|Return|$             &        8.21&         ***&        8.21&         ***&        8.21&         ***&        8.21&         ***&        9.44&         ***&        9.44&         ***\\
                    &      (7.84)&            &      (7.84)&            &      (7.84)&            &      (7.84)&            &      (6.98)&            &      (6.98)&            \\
$Volume$            &       -0.04&         ***&       -0.04&         ***&       -0.04&         ***&       -0.04&         ***&        0.28&         ***&        0.28&         ***\\
                    &     (-6.02)&            &     (-6.02)&            &     (-6.02)&            &     (-6.02)&            &      (7.72)&            &      (7.72)&            \\
$Volatility$             &        3.24&         ***&        3.24&         ***&        3.24&         ***&        3.24&         ***&      -17.09&         ***&      -17.09&         ***\\
                    &      (5.44)&            &      (5.44)&            &      (5.44)&            &      (5.44)&            &     (-6.58)&            &     (-6.58)&            \\
\midrule
$ R^2$              &        0.36&            &        0.17&            &        0.21&            &        0.27&            &        0.09&            &        0.19&            \\
$ Observations$             &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_slip_usdc_eth_005_pres.tex <==
\begin{tabularx}{\textwidth}{l *{4}{R@{ }l}} \\
\toprule
 \multicolumn{9}{l}{ \textbf{Panel A: ETH/USDC 0.05\%}} \\  \hline 
 & \multicolumn{8}{c}{Slippage}  \\ 
 & Total & & \$1K cutoff & & \$5K cutoff & & \$10K cutoff&  \\ 
& (1) & & (2) & & (3) & & (4) &   \\ 
\midrule
$Polygon$           &       18.38&         ***&      -20.12&         ***&      -19.92&         ***&      -19.61&         ***    \\
                    &      (6.45)&            &     (-5.72)&            &     (-5.67)&            &     (-5.59)&               \\
$Polygon\cdot Large$&            &            &       57.75&         ***&       68.93&         ***&       85.47&         ***    \\
                    &            &            &     (26.72)&            &     (26.69)&            &     (26.65)&              \\
$Large$             &            &            &        3.99&         ***&        4.76&         ***&        5.90&         ***   \\
                    &            &            &     (29.75)&            &     (29.75)&            &     (29.75)&            \\
$Size$              &        0.12&         ***&            &            &            &            &            &          \\
                    &     (26.40)&            &            &            &            &            &            &    \\

\midrule
$ R^2$              &        0.36&            &        0.17&            &        0.21&            &        0.27&         \\
$ Obs.$             &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&     \\
%$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&              \\
%$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&                 \\
\bottomrule
\end{tabularx}


==> files_v1/estimation_slip_usdc_eth_030.tex <==
\begin{tabularx}{\textwidth}{l *{6}{R@{ }l}} \\
\toprule
 \multicolumn{13}{l}{ \textbf{Panel B: ETH/USDC 0.3\%}} \\  \hline 
 & \multicolumn{8}{c}{$Slippage$} & \multicolumn{4}{c}{$ExecutionCost$}  \\ 
 & Total & & \$1K cutoff & & \$5K cutoff & & \$10K cutoff& & Total & & \$5K cutoff&  \\ 
& (1) & & (2) & & (3) & & (4) & & (5) & & (6) &  \\ 
\midrule
$Polygon$           &       16.48&         ***&      -20.69&         ***&      -20.49&         ***&      -20.19&         ***&     -128.27&         ***&     -421.83&         ***\\
                    &      (8.39)&            &     (-7.69)&            &     (-7.62)&            &     (-7.53)&            &     (-6.38)&            &    (-12.67)&            \\
$Polygon\cdot Large$&            &            &       55.76&         ***&       66.56&         ***&       82.52&         ***&            &            &      528.40&         ***\\
                    &            &            &     (26.24)&            &     (26.21)&            &     (26.17)&            &            &            &     (17.41)&            \\
$Large$             &            &            &        5.51&         ***&        6.57&         ***&        8.14&         ***&            &            &     -455.60&         ***\\
                    &            &            &     (58.03)&            &     (58.03)&            &     (58.03)&            &            &            &    (-15.15)&            \\
$Size$              &        0.12&         ***&            &            &            &            &            &            &       -0.06&         ***&            &            \\
                    &     (28.18)&            &            &            &            &            &            &            &     (-4.70)&            &            &            \\
\midrule
$ R^2$              &        0.39&            &        0.18&            &        0.23&            &        0.29&            &        0.09&            &        0.18&            \\
$ Observations$             &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            &    18,921,636&            \\
$ HourFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            \\
$ DayFE$             &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            &    Yes&            \\
\bottomrule
\end{tabularx}


==> files_v1/pool_stats.tex <==
\begin{tabular}{|cccc|}
    \hline
        \textbf{Uniswap v3 ETH/USDC 0.05\%} & \textbf{Ethereum} & \textbf{Polygon} & \textbf{t-stat}\\ \hline
        volume (\$M) & 30.92 & 1.38 & (73.10) \\
        minted (\$M) & 45.23 & 14.86 & (15.52) \\
        burned (\$M) & 45.19 & 14.86 & (15.51) \\
        TVL (\$M) & 199.22 & 13.01 & (378.94) \\
        volume/TVL & 16.21\% & 11.72\% & (15.24) \\
        minted/TVL & 22.92\% & 99.81\% & (-20.09) \\
        burned/TVL & 22.95\% & 99.79\% & (-20.08) \\
        (minted+burned)/volume & 45.87\% & 200\% & (-20.09) \\ \hline
\end{tabular}

==> files_v1/pool_stats_2.tex <==
\begin{tabular}{|cccc|}
    \hline
        \textbf{Uniswap v3 ETH/USDC 0.05\%} & \textbf{Ethereum} & \textbf{Polygon} & \textbf{t-stat}\\ \hline
        |mean| & 1122 & 854 & (16.29) \\
        variance & 14090000 & 12200000 & (12.39) \\
        skewness & -0.79 & 0.24 & (-16.58) \\
        kurtosis & -1.84 & -0.91 & (-11.81) \\ \hline
\end{tabular}

==> files_v1/reg_slippage_final.tex <==
\begin{tabular}{|ccccccccc|}
    \hline
    \textbf{slip}          & \multicolumn{4}{c}{\textbf{ETH}}            & \multicolumn{4}{c|}{\textbf{BTC}}          \\
                  & (1)        &     & (2)       &     & (3)       &     & (4)       &     \\ \hline
    uni\_v2       & 0.0105     & *** & -2.49e-5 &     & 2.137  & *** & 0.0171 &     \\
                  & (41.74)    &     & (-0.13)   &     & (76.35)   &     & (1.07)    &     \\
    uni\_v2*large &            &     & 0.0179  & *** &           &     & 3.611  & *** \\
                  &            &     & (85.11)   &     &           &     & (98.21)   &     \\
    uni\_v3       & -0.0008 & *** & -2.63e-5 &     & 0.0107  &     & 0.0068  &     \\
                  & (-8.13)    &     & (-0.31)   &     & (0.69)    &     & (0.43)    &     \\
    uni\_v3*large &            &     & -0.0012 & *** &           &     & 0.0068  & *** \\
                  &            &     & (-18.21)  &     &           &     & (24.35)   &     \\
    large         &            &     & 0.0025  & *** &           &     & 0.0016 & *** \\
                  &            &     & (31.02)   &     &           &     & (34.29)   &     \\
    size          & 0.0036   & *** &           &     & 0.496  & *** &           &     \\
                  & (84.31)    &     &           &     & (131.22)  &     &           &     \\
    buy           & -0.0002 & *** & -0.0002 & *** & 1.193  & *** & 1.193  & *** \\
                  & (-8.53)    &     & (-8.53)   &     & (87.89)   &     & (87.89)   &     \\
    volume        & -3.51e-8  &     & -3.51e-8 &     & 3.57e-6  &     & 3.57e-6  &     \\
                  & (-0.26)    &     & (-0.26)   &     & (0.43)    &     & (0.43)    &     \\
    volatility    & 0.0119    & **  & 0.0119  & **  & 0.2090  &     & 0.2090  &     \\
                  & (2.42)     &     & (2.42)    &     & (0.85)    &     & (0.85)    &     \\
    $|\text{return}|$      & 0.0012  &     & 0.0013  &     & 0.2481 &     & 0.2481 &     \\
                  & (0.57)     &     & (0.57)    &     & (1.32)    &     & (1.32)    &     \\
    constant      & -0.0035   & *** & -0.0003 & **  & -1.266 & *** & -0.6197 & *** \\
                  & (-23.41)   &     & (-2.12)   &     & (-58.86)  &     & (-34.91)  &     \\ \hline
    N             & 41492      &     & 41492     &     & 41676     &     & 41676     &     \\
    R2            & 0.52       &     & 0.27      &     & 0.26      &     & 0.21      &     \\
    Weekday FE    & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\
    Month FE      & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\ \hline
\end{tabular}

==> files_v1/reg_slippage_gas_final.tex <==
\begin{tabular}{|ccccccccc|}\hline
    \textbf{slip + gas}          & \multicolumn{4}{c}{\textbf{ETH}}            & \multicolumn{4}{c|}{\textbf{BTC}}          \\
                  & (1)        &     & (2)       &     & (3)       &     & (4)       &     \\ \hline
    uni\_v2       & 0.0351  & *** & 0.0515 & *** & 2.159  & *** & 0.0668  & *** \\
                  & (11.56)   &     & (11.95)   &     & (74.08)   &     & (3.80)    &     \\
    uni\_v2*large &           &     & -0.028 & *** &           &     & 3.565  & *** \\
                  &           &     & (-10.30)  &     &           &     & (99.86)   &     \\
    uni\_v3       & 0.0208  & *** & 0.0485  & *** & 0.0334  & **  & 0.0564  & *** \\
                  & (11.24)   &     & (14.73)   &     & (1.99)    &     & (3.26)    &     \\
    uni\_v3*large &           &     & -0.0472 & *** &           &     & -0.0392 & *** \\
                  &           &     & (-17.63)  &     &           &     & (-14.56)  &     \\
    large         &           &     & 0.0025  & *** &           &     & 0.0016  & *** \\
                  &           &     & (31.02)   &     &           &     & (34.29)   &     \\
    size          & 0.0012  & *** &           &     & 0.494  & *** &           &     \\
                  & (7.50)    &     &           &     & (132.33)  &     &           &     \\
    buy           & -0.0002 & *** & -0.0002 & *** & 1.193  & *** & 1.193  & *** \\
                  & (-8.53)   &     & (-8.53)   &     & (87.89)   &     & (87.89)   &     \\
    volume        & 3.87e-6  & **  & 3.87e-6  & **  & 5.38e-6  &     & 5.38e-6  &     \\
                  & (2.21)    &     & (2.21)    &     & (0.61)    &     & (0.61)    &     \\
    volatility    & -0.1003 &     & -0.1003 &     & 0.1604  &     & 0.1603  &     \\
                  & (-1.42)   &     & (-1.42)   &     & (0.68)    &     & (0.68)    &     \\
    $|\text{return}|$      & 0.0369  & **  & 0.0369  & **  & 0.2596  &     & 0.2596  &     \\
                  & (2.32)    &     & (2.32)    &     & (1.38)    &     & (1.38)    &     \\
    constant      & -0.0029 & **  & -0.0028 & **  & -1.265 & *** & -0.6222 & *** \\
                  & (-2.23)   &     & (-2.06)   &     & (-57.45)  &     & (-33.87)  &     \\ \hline
    N             & 41492     &     & 41492     &     & 41676     &     & 41676     &     \\
    R2            & 0.078     &     & 0.16      &     & 0.26      &     & 0.21      & \\
    Weekday FE    & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\
    Month FE      & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\ \hline
\end{tabular}

==> files_v1/reg_slippage_gas_polygon_final.tex <==
\begin{tabular}{|ccccccccc|}
    \hline
    \textbf{slip + gas}          & \multicolumn{4}{c}{\textbf{ETH}}            & \multicolumn{4}{c|}{\textbf{BTC}}          \\
                  & (1)        &     & (2)       &     & (3)       &     & (4)       &     \\ \hline
    uni\_v2               & 0.0306  & *** & 0.0471  & *** & 2.222  & *** & 0.1363  & *** \\
                          & (13.98)   &     & (13.23)   &     & (42.84)   &     & (2.91)    &     \\
    uni\_v2*large         &           &     & -0.028 & *** &           &     & 3.565  & *** \\
                          &           &     & (-10.30)  &     &           &     & (99.86)   &     \\
    uni\_v3               & 0.0188   & *** & 0.0465  & *** & 0.0955  & **  & 0.1251  & *** \\
                          & (12.39)   &     & (15.41)   &     & (2.11)    &     & (2.71)    &     \\
    uni\_v3*large         &           &     & -0.0472 & *** &           &     & -0.0392 & *** \\
                          &           &     & (-17.63)  &     &           &     & (-14.56)  &     \\
    uni\_v3*polygon       & 0.0102  & *** & -0.0452 & *** & 1.16   & *** & -0.0462 & *** \\
                          & (10.62)   &     & (-18.14)  &     & (14.09)   &     & (-13.29)  &     \\
    uni\_v3*polygon*large &           &     & 0.0944  & *** &           &     & 1.909  & *** \\
                          &           &     & (28.47)   &     &           &     & (12.32)   &     \\
    large                 &           &     & 0.0025  & *** &           &     & 0.0016  & *** \\
                          &           &     & (31.02)   &     &           &     & (34.29)   &     \\
    size                  & 0.0068  & *** &           &     & 0.587  & *** &           &     \\
                          & (47.08)   &     &           &     & (43.13)   &     &           &     \\
    buy                   & -0.0031 & *** & -0.0031 & *** & 1.203  & *** & 1.250  & *** \\
                          & (-11.40)  &     & (-11.40)  &     & (36.76)   &     & (40.17)   &     \\
    volume                & 6.78e-7  &     & 6.78e-7  &     & 3.80e-5  &     & 4.14e-5  & *   \\
                          & (0.62)    &     & (0.62)    &     & (1.59)    &     & (1.71)    &     \\
    volatility            & 0.0250  &     & 0.025  &     & -0.6422 &     & -0.7829 &     \\
                          & (0.64)    &     & (0.64)    &     & (-0.71)   &     & (-0.84)   &     \\
    $|\text{return}|$              & 0.0322  & **  & 0.0322  & **  & 0.11  &     & 0.1185  &     \\
                          & (2.38)    &     & (2.38)    &     & (0.20)    &     & (0.21)    &     \\
    constant              & -0.0088 & *** & -0.0014 &     & -1.442 & *** & -0.7041 & *** \\
                          & (-7.68)   &     & (-1.16)   &     & (-21.76)  &     & (-13.23)  &     \\ \hline
    N                     & 55384     &     & 55384     &     & 53162     &     & 53162     &     \\
    R2                    & 0.16      &     & 0.16      &     & 0.29      &     & 0.19      & \\ 
    Weekday FE    & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\
    Month FE      & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\ \hline
\end{tabular}


==> files_v1/reg_slippage_polygon_final.tex <==
\begin{tabular}{|ccccccccc|}\hline
    \textbf{slip}          & \multicolumn{4}{c}{\textbf{ETH}}            & \multicolumn{4}{c|}{\textbf{BTC}}          \\
                  & (1)        &     & (2)       &     & (3)       &     & (4)       &     \\ \hline
    uni\_v2               & 0.0071  & *** & -0.0035 & *** & 2.2   & *** & 0.0874  & *   \\
                          & (9.02)    &     & (-4.57)   &     & (42.90)   &     & (1.90)    &     \\
    uni\_v2*large         &           &     & 0.018  & *** &           &     & 3.611  & *** \\
                          &           &     & (85.11)   &     &           &     & (98.22)   &     \\
    uni\_v3               & -0.0023 & *** & -0.0016 & *** & 0.0736  &     & 0.0762  & *   \\
                          & (-6.93)   &     & (-4.79)   &     & (1.64)    &     & (1.67)    &     \\
    uni\_v3*large         &           &     & -0.0012 & *** &           &     & 0.0068  & *** \\
                          &           &     & (-18.21)  &     &           &     & (24.35)   &     \\
    uni\_v3*polygon       & 0.0268  & *** & -0.0018 & *** & 1.178  & *** & -0.0007 &     \\
                          & (38.88)   &     & (-4.29)   &     & (14.26)   &     & (-0.35)   &     \\
    uni\_v3*polygon*large &           &     & 0.0489  & *** &           &     & 1.862  & *** \\
                          &           &     & (41.17)   &     &           &     & (12.08)   &     \\
    large                 &           &     & 0.0025  & *** &           &     & 0.0016  & *** \\
                          &           &     & (31.02)   &     &           &     & (34.29)   &     \\
    size                  & 0.0087    & *** &           &     & 0.589     & *** &           &     \\
                          & (65.17)   &     &           &     & (43.19)   &     &           &     \\
    buy                   & -0.003 & *** & -0.003 & *** & 1.203  & *** & 1.250  & *** \\
                          & (-11.40)  &     & (-11.40)  &     & (36.75)   &     & (40.17)   &     \\
    volume                & -2.52e-6 & *** & -2.52e-6 & *** & 3.66e-5  &     & 4.00e-5  & *   \\
                          & (-4.55)   &     & (-4.55)   &     & (1.54)    &     & (1.67)    &     \\
    volatility            & 0.1015  & *** & 0.1015  & *** & -0.6045 &     & -0.7439 &     \\
                          & (6.32)    &     & (6.32)    &     & (-0.67)   &     & (-0.80)   &     \\
    $|\text{return}|$              & 0.005  &     & 0.005  &     & 0.0994    &     & 0.1074  &     \\
                          & (0.73)    &     & (0.73)    &     & (0.18)    &     & (0.19)    &     \\
    constant              & -0.0086 & *** & 0.0013  & **  & -1.442 & *** & -0.7018  & *** \\
                          & (-16.60)  &     & (2.61)    &     & (-21.84)  &     & (-13.27)  &     \\ \hline
    N                     & 55384     &     & 55384     &     & 53162     &     & 53162     &     \\
    R2                    & 0.44      &     & 0.22      &     & 0.29      &     & 0.19      & \\ 
    Weekday FE    & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\
    Month FE      & Yes        &     & Yes       &     & Yes       &     & Yes       &     \\ \hline
\end{tabular}

==> files_v1/summary_stat.tex <==
\begin{tabular}{|lccccccc|}
    \hline
        & \textbf{Mean} & \textbf{SD} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \textbf{Min} & \textbf{Max} \\ \hline
        \textbf{BTC} & & & & & & & \\
        Binance & 8.925 & 19.21 & 0.001260 & 0.1633 & 3.910 & 0.001057 & 91.25 \\
        Uniswap v3 (Ethereum) & 47.05 & 98.34 & 0.1021 & 1.822 & 27.24 & 0.003257 & 494.3 \\
        Uniswap v3 (Polygon) & 13360 & 68110 & 3.455 & 43.52 & 586.1 & 0.1109 & 1185000 \\
       % Uniswap v2 & 22750 & 62720 & 96.46 & 1593 & 9268 & 3.219 & 331900 \\ \hline
        \textbf{ETH} & & & & & & & \\
        Binance & 14.34 & 31.80 & 0.01797 & 0.4761 & 6.030 & 0.01328 & 162.1 \\
        Uniswap v3 (Ethereum) & 7.335 & 15.46 & 0.01531 & 0.2754 & 4.242 & 0.0005160 & 77.25 \\
        Uniswap v3 (Polygon) & 494.3 & 1741 & 0.4013 & 7.180 & 113.8 & 0.01304 & 12930 \\
       % Uniswap v2 & 120.0 & 238.4 & 0.2876 & 5.071 & 74.82 & 0.009590 & 965.6 \\ \hline
\end{tabular}

==> files_v1/t_stat_slippage_btc.tex <==
\begin{tabular}{|cccccc|}
    \hline
        \textbf{Trade size (\$)} & \textbf{Uniswap v3 (Ethereum)} & \textbf{Uniswap v2} & \textbf{t-stat} & \textbf{Binance} & \textbf{t-stat} \\ \hline
        100 & 0.003754 & 3.289 & (-89.06) & 0.01619 & (-2.78) \\
        1K & 0.03754 & 32.84 & (-89.18) & 0.02138 & (2.93) \\
        10K & 0.3753 & 323.5 & (-90.10) & 0.08853 & (17.09) \\
        100K & 3.750 & 2873 & (-74.87) & 0.6823 & (28.28) \\
        1M & 37.27 & 20250 & (-26.20) & 5.209 & (32.53) \\
        10M & 377.8 & 169300 & (-17.72) & 71.38 & (30.37) \\ \hline
\end{tabular}

==> files_v1/t_stat_slippage_eth.tex <==
\begin{tabular}{|cccccc|}
    \hline
        \textbf{Trade size (\$)} & \textbf{Uniswap v3 (Ethereum)} & \textbf{Uniswap v2} & \textbf{t-stat} & \textbf{Binance} & \textbf{t-stat} \\ \hline
        100 & 0.0005800 & 0.009542 & (-114.58) & 0.03717 & (-8.69) \\
        1K & 0.005797 & 0.09542 & (-114.58) & 0.05504 & (-6.94) \\
        10K & 0.05797 & 0.9542 & (-114.58) & 0.1782 & (-6.33) \\
        100K & 0.5796 & 9.537 & (-114.65) & 1.123 & (-8.54) \\
        1M & 5.779 & 94.95 & (-115.27) & 9.112 & (-8.13) \\
        10M & 58.10 & 911.7 & (-112.80) & 122.3 & (-17.36) \\ \hline
\end{tabular}

==> files_v1/t_stat_slippage_gas_btc.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
        Trade size (\$) & Uniswap v3 (Ethereum) & Uniswap v2 & t-stat & Binance & t-stat \\ \hline
        100 & 5510 & 5513 & (-0.011) & 0.01619 & (26.93) \\
        1K & 551.1 & 583.9 & (-1.13) & 0.02138 & (26.93) \\
        10K & 55.48 & 379.6 & (-58.99) & 0.08852 & (27.07) \\
        100K & 9.270 & 2879 & (-74.71) & 0.6823 & (36.89) \\
        1M & 37.83 & 20250 & (-26.20) & 5.209 & (33.13) \\
        10M & 377.8 & 169300 & (-17.72) & 71.38 & (30.37) \\ \hline
\end{tabular}

==> files_v1/t_stat_slippage_gas_eth.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
    Trade size (\$) & Uniswap v3 (Ethereum) & Uniswap v2 & t-stat & Binance & t-stat \\ \hline
    100 & 5510 & 5510 & (-0.000031) & 0.03717 & (26.75) \\
    1K & 551.0 & 551.1 & (-0.0031) & 0.05504 & (26.75) \\
    10K & 55.16 & 56.06 & (-0.31) & 0.1782 & (26.69) \\
    100K & 6.095 & 15.07 & (-30.40) & 1.123 & (22.95) \\
    1M & 6.338 & 95.51 & (-115.65) & 9.112 & (-6.75) \\
    10M & 58.15 & 911.8 & (-112.80) & 122.3 & (-17.34) \\ \hline
\end{tabular}

==> files_v1/table1.tex <==
\begin{tabular}{cccc}    \hline
    \textbf{Pool} & \textbf{Volume 24h (\$M)} & \textbf{TVL (\$M)} & \textbf{Volume/TVL} \\ \hline
    ETH/USDC 0.05\% & & & \\
    Ethereum & 588.74 & 174.14 & 3.38 \\
    Polygon & 33.53 & 10.84 & 3.09 \\ \hline
    ETH/USDC 0.3\% & & & \\
    Ethereum & 76.84 & 201.01 & 0.38 \\
    Polygon & 1.26 & 2.27 & 0.56 \\ \hline
    ETH/USDT 0.3\% & & & \\
    Ethereum & 28.32 & 81.57 & 0.35 \\
    Polygon & 0.13 & 0.34 & 0.38 \\ 
    \hline \end{tabular}

==> files_v1/table2a.tex <==
\begin{tabular}{cccccc}
    \hline
    \textbf{Pool} & \textbf{Mean (\$K)} & \textbf{SD} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} \\ \hline
    ETH/USDC 0.05\% \\
    Ethereum & 78.17 & 267.28 & 0.85 & 5.00 & 48.44 \\
    Polygon & 2.49 & 5.01 & 0.11 & 0.93 & 3.00 \\ \hline
    ETH/USDC 0.3\% \\
    Ethereum & 134.19 & 262.52 & 1.87 & 44.06 & 173.24\\
    Polygon & 1.84 & 3.55 & 0.40 & 0.92 & 1.94 \\ \hline
    ETH/USDT 0.3\% \\
    Ethereum & 68.11 & 160.97 & 1.62 & 30.04 & 87.26 \\
    Polygon & 0.35 & 0.64 & 0.09 & 0.19 & 0.40 \\ \hline
\end{tabular}

==> files_v1/table2b.tex <==
\begin{tabular}{ccccc}
    \hline
    \textbf{Pool} & \textbf{Daily trades} & \textbf{Daily buys} & \textbf{Daily sells} & \textbf{Delta (s)} \\ \hline
    ETH/USDC 0.05\% \\
    Ethereum & 7545	&3906	&3639	&23.03 \\
    Polygon &13502&	6915	&6582	&10.03\\ \hline
    ETH/USDC 0.3\% \\
    Ethereum & 573&	299&	274&	182.20\\
    Polygon & 685	&349&	335&	146.32 \\ \hline
    ETH/USDT 0.3\% \\
    Ethereum & 416&	211	&206&	234.54 \\
    Polygon & 366&	173&	193&	252.20 \\ \hline
\end{tabular}

==> files_v1/table3.tex <==
\begin{tabular}{cccccc}
    \hline
    & \textbf{Mean} & \textbf{SD} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} \\ \hline
    Slippage (bp) \\
    Ethereum & 5.93	&14.92	&0.02	&0.29	&4.00 \\
    Polygon & 700.90	&2066.06	&0.66	&9.35	&118.73\\ \hline
    Volume 24h (\$M) \\
    Ethereum & 231.30&	319.64&	26.08&	68.17&	382.89\\
    Polygon & 11.64	&19.19	&0.15	&1.03	&20.74\\ \hline
    Volatility 24h (\%) & 4.06	&1.99	&2.81	&3.72	&4.74\\ 
    Return 1min (bp) & -0.01&	11.91&	-4.73	&0.00	&4.63 \\ \hline
\end{tabular}

==> files_v1/table3a.tex <==
\begin{tabular}{ccccc}
\hline
& \multicolumn{2}{c}{\textbf{$Slippage$ (bp)}} & \multicolumn{2}{c}{\textbf{$ExecutionCost$ (bp)}} \\ 
\textbf{Trade size (\$)}& \textbf{Ethereum} & \textbf{Polygon} & \textbf{Ethereum} & \textbf{Polygon} \\ \hline
100     & 0.0015  & 0.0202   & 1400.0015 & 1.0202   \\
500     & 0.0073  & 0.1009   & 280.0073  & 0.3009   \\
1000    & 0.0147  & 0.2018   & 140.0147  & 0.3018   \\
5000    & 0.0734  & 1.0079   & 28.0734   & 1.0279   \\
10000   & 0.1467  & 2.0133   & 14.1467   & 2.0233   \\
50000   & 0.7331  & 9.9879   & 3.5331    & 9.9899   \\
100000  & 1.4645  & 19.8670  & 2.8645    & 19.8680  \\
500000  & 7.2618  & 100.1648 & 7.5418    & 100.1650 \\
1000000 & 14.4243 & 206.7951 & 14.5643   & 206.7952 \\ \hline
\end{tabular}

==> files_v1/table3b.tex <==
\begin{tabular}{ccccc}
\hline
& \multicolumn{2}{c}{\textbf{$Slippage$ (bp)}} & \multicolumn{2}{c}{\textbf{$ExecutionCost$ (bp)}} \\ 
\textbf{Trade size (\$)}& \textbf{Ethereum} & \textbf{Polygon} & \textbf{Ethereum} & \textbf{Polygon} \\ \hline
100     & 0.0020  & 0.0203   & 1400.0020 & 1.0203   \\
500     & 0.0100  & 0.1014   & 280.0100  & 0.3014   \\
1000    & 0.0201  & 0.2027   & 140.0201  & 0.3027   \\
5000    & 0.1003  & 1.0129   & 28.1003   & 1.0329   \\
10000   & 0.2007  & 2.0246   & 14.2007   & 2.0346   \\
50000   & 1.0032  & 10.0876  & 3.8032    & 10.0896  \\
100000  & 2.0059  & 20.1401  & 3.4059    & 20.1411  \\
500000  & 10.0024 & 102.0050 & 10.2824   & 102.0052 \\
1000000 & 19.9350 & 210.7848 & 20.0750   & 210.7849 \\ \hline
\end{tabular}

==> files_v1/table3c.tex <==
\begin{tabular}{ccccc}
\hline
& \multicolumn{2}{c}{\textbf{$Slippage$ (bp)}} & \multicolumn{2}{c}{\textbf{$ExecutionCost$ (bp)}} \\ 
\textbf{Trade size (\$)}& \textbf{Ethereum} & \textbf{Polygon} & \textbf{Ethereum} & \textbf{Polygon} \\ \hline
100     & 0.0062  & 1.6693    & 1400.0062 & 2.6693    \\
500     & 0.0308  & 8.3769    & 280.0308  & 8.5769    \\
1000    & 0.0616  & 16.7965   & 140.0616  & 16.8965   \\
5000    & 0.3081  & 86.4631   & 28.3081   & 86.4831   \\
10000   & 0.6161  & 185.6604  & 14.6161   & 185.6704  \\
50000   & 3.0801  & 1099.0471 & 5.8801    & 1099.0491 \\
100000  & 6.1609  & 2055.2035 & 7.5609    & 2055.2045 \\
500000  & 30.8244 & 6593.3406 & 31.1044   & 6593.3408 \\
1000000 & 61.7460 & 8191.2155 & 61.8860   & 8191.2156 \\ \hline
\end{tabular}

==> files_v1/table4a.tex <==
\begin{tabular}{ccccccc}
    \hline
    \textbf{Pool} & \multicolumn{6}{c}{\textbf{Liquidity concentration (\%)}} \\ 
				  & \multicolumn{2}{c}{\textbf{1\%}} & \multicolumn{2}{c}{\textbf{2\%}} & \multicolumn{2}{c}{\textbf{10\%}}   \\ \hline
    ETH/USDC 0.05\% \\
    Ethereum & 5.21	&&9.82	&&35.02 &\\
    Polygon &5.69&&	10.75	&&37.97 &\\   
    Difference &0.48&***&	0.93&***&2.95&***\\
    t-stat &(-51.04)&&(-57.36)&	&(-70.70)&\\\hline
    ETH/USDC 0.3\% \\
    Ethereum & 2.73&&	5.42&&	23.98&\\
    Polygon & 5.09 &&9.89&&	36.68&\\
    Difference &2.36&***&	4.47&***&12.70&***\\
    t-stat &(-290.00)&&(-310.00)&	&(-320.00)&\\\hline
    ETH/USDT 0.3\% \\
    Ethereum & 2.44&&	4.87 &&22.47 & \\
    Polygon & 3.70&&	7.30&&	27.40 & \\
    Difference &1.25&***&	2.43&***&4.93&***\\
    t-stat &(-130.00)&&(-140.00)&	&(-110.00)&\\\hline
\end{tabular}

==> files_v1/table4b.tex <==
\begin{tabular}{cccccccc}
    \hline
    \textbf{Pool} & \textbf{Mints} & \textbf{Delta} & \textbf{Minted} & \textbf{Burns} & \textbf{Delta} & \textbf{Burned} & \textbf{Intensity} \\
    & \textbf{(\#/day)} & \textbf{(min)} & \textbf{(\$M/day)} & \textbf{(\#/day)} & \textbf{(min)} & \textbf{(\$M/day)} & \textbf{(\%)} \\\hline
    ETH/USDC 0.05\% \\
    Ethereum & 83.94 & 17.16 & 29.12 & 32.83 & 43.86 & 15.71 & 17.01 \\
    Polygon & 512.95 & 2.81 & 35.46 & 324.36 & 4.44 & 35.15 & 35.36 \\  
    Difference &  -429.01 & 14.35 & -6.33 & -291.54 & 39.42 & -19.44 & -18.26 \\
    t-stat & (-27.54) & & (-0.70) & (-24.19) & & (-2.16) & (-65.81) \\\hline
    ETH/USDC 0.3\% \\
    Ethereum & 97.83 & 14.72 & 9.11 & 22.79 & 63.19 & 4.67 & 8.68 \\
    Polygon & 92.42 & 15.58 & 0.43 & 43.31 & 33.25 & 0.21 & 19.33 \\  
    Difference & 5.41 & -0.86 & 8.68 & -20.52 & 29.94 & 4.46 & -10.66 \\
    t-stat & (0.90) & & (16.59) & (-8.01) & & (12.95) & (-39.07) \\\hline
    ETH/USDT 0.3\% \\
    Ethereum & 13.48 & 106.82 & 1.97 & 3.07 & 469.06 & 0.57 & 12.21 \\
    Polygon & 11.86 & 121.42 & 0.04 & 6.74 & 213.65 & 0.02 & 18.65 \\  
    Difference & 1.62 & -14.59 &  1.93 & -3.67 & 255.41 & 0.55 & -6.44 \\
    t-stat & (2.69) & & (9.01) & (-5.89) & & (8.10) & (-8.24) \\\hline
\end{tabular}

==> files_v1/table4b_pres.tex <==
\begin{tabular}{cccccc}
    \hline
    \textbf{Pool} & \textbf{Mints} &  \textbf{Minted} & \textbf{Burns} &  \textbf{Burned} & \textbf{Intensity} \\
    & \textbf{(\#/day)} & \textbf{(\$M/day)} & \textbf{(\#/day)} & \textbf{(\$M/day)} & \textbf{(\%)} \\\hline
    ETH/USDC 0.05\% \\
    Ethereum & 83.94 & 29.12 & 32.83 &  15.71 & 17.01 \\
    Polygon & 512.95 & 35.46 & 324.36 &  35.15 & 35.36 \\  
    Difference &  -429.01 &  -6.33 & -291.54 &  -19.44 & -18.26 \\
    t-stat & (-27.54) &  (-0.70) & (-24.19) &  (-2.16) & (-65.81) \\\hline
    ETH/USDC 0.3\% \\
    Ethereum & 97.83 & 9.11 & 22.79 &  4.67 & 8.68 \\
    Polygon & 92.42 &  0.43 & 43.31 &  0.21 & 19.33 \\  
    Difference & 5.41 &  8.68 & -20.52 & 4.46 & -10.66 \\
    t-stat & (0.90) & (16.59) & (-8.01) & (12.95) & (-39.07) \\\hline
    ETH/USDT 0.3\% \\
    Ethereum & 13.48 &  1.97 & 3.07 &  0.57 & 12.21 \\
    Polygon & 11.86 &  0.04 & 6.74 &  0.02 & 18.65 \\  
    Difference & 1.62 &  1.93 & -3.67 & 0.55 & -6.44 \\
    t-stat & (2.69) &  (9.01) & (-5.89) &  (8.10) & (-8.24) \\\hline
\end{tabular}

==> files_v1/table5_sumstat.tex <==
\begin{tabular}{cccccc}
    \hline
    & \textbf{Mean} & \textbf{SD} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} \\ \hline
    Slippage (bp) \\
    Ethereum & 5.93	&14.92	&0.02	&0.29	&4.00 \\
    Polygon & 700.90	&2066.06	&0.66	&9.35	&118.73\\ \hline
    Volume 24h (\$M) \\
    Ethereum & 231.30&	319.64&	26.08&	68.17&	382.89\\
    Polygon & 11.64	&19.19	&0.15	&1.03	&20.74\\ \hline
    Volatility 24h (\%) & 4.06	&1.99	&2.81	&3.72	&4.74\\ 
    Return 1min (bp) & -0.01&	11.91&	-4.73	&0.00	&4.63 \\ \hline
\end{tabular}

==> files_v1/table6.tex <==
\begin{tabularx}{\textwidth}{cRlRlRl}
    \hline
    \textbf{Pool} & \multicolumn{2}{c}{\textbf{Position}} & \multicolumn{2}{c}{\textbf{Position}} & \multicolumn{2}{c}{\textbf{Position}}   \\ 
	 & \multicolumn{2}{c}{\textbf{gap (\%)}} & \multicolumn{2}{c}{\textbf{length (\%)}} & \multicolumn{2}{c}{\textbf{concentration (\%)}}   \\ 
	\hline
    ETH/USDC 0.05\% \\
    Ethereum & 2.65	&& 19.91 && 36.30 &\\
    Polygon & 1.99 && 14.27 && 47.82 &\\   
    Difference & 0.66 &***& 5.64 &***& -11.52 &***\\
    t-stat & (26.13) &  & (29.11) &  & (-37.94) & \\\hline
    ETH/USDC 0.3\% \\
    Ethereum & 3.65	&& 70.88 && 12.38 &\\
    Polygon & 2.94 && 23.67 && 25.85 &\\   
    Difference & 0.71 & ***& 47.21 &***& -13.47 &***\\
    t-stat & (17.50) & & (110.44) &  & (-50.77) & \\\hline
    ETH/USDT 0.3\% \\
    Ethereum & 3.89	&& 68.81 && 12.79 &\\
    Polygon & 3.26 && 34.65 && 18.27 &\\   
    Difference & 0.63 &***& 34.16 &*** & -5.48 &***\\
    t-stat & (5.92) &  & (29.81) & & (-9.16) & \\\hline
\end{tabularx}

==> files_v1/trades_stat.tex <==
\begin{tabular}{ccc}
    \hline
    \textbf{Uniswap v3 ETH/USDC 0.05\%} & \textbf{Ethereum} & \textbf{Polygon}\\ \hline
    mean & 118300 & 2738\\
    SD & 251700 & 3976 \\
    25\% & 2845 & 195.0 \\
    50\% & 14300 & 1154 \\
    75\% & 99760 & 3555 \\
    min & 60.49 & 1.793 \\
    max & 1521000 & 22840 \\ \hline
\end{tabular}

==> files_v1/variables.tex <==
\begin{tabular}{lp{9cm}l}\hline
Variable & Description & Source \\\hline

$Buy$& A variable that takes the value 1 if the trade is a buy of tokens X with tokens Y, and zero otherwise. & BigQuery\\

$ExecutionCost$ & Total execution cost, computed as the sum of $Slippage$ and gas fees relative to $Size$. & BigQuery, Etherscan\\

$Intensity$& Repositioning intensity of liquidity providers, measured as $1-\frac{\lvert Minted-Burned \rvert}{Minted+Burned}$ within a given interval (5min, 10min, etc.), $Minted$ ($Burned$) being the \$ value of the minted (burned) liquidity. & BigQuery\\

$Large$&A variable that takes the value 1 if the size of the trade exceeds a specified cutoff (\$1K/\$5K/\$10K), and zero otherwise. &\\

$LiquidityConcentration$&Market depth within 1\%/2\%/10\% of $p_{mkt}$, divided by $TVL$. Market depth within x\% of $p_{mkt}$ is computed as the \$ value of the liquidity between $\frac{p_{mkt}}{1+x\%}$ and $p_{mkt} \cdot (1+x\%)$ & BigQuery\\

$p_{mid}$ & Mid price of a position, computed as $\sqrt{p_{lower} \cdot p_{upper}}$. & BigQuery\\

$p_{mkt}$&On DEXs: price of the pool. On CEXs: mid price of the limit order book.& BigQuery\\

$Polygon$&A variable that takes the value 1 if the transaction takes place on Polygon, and zero otherwise. & BigQuery\\

$PositionConcentration$& Concentration of a position around $p_{mkt}$, computed and scaled as $1-1.0001^{\frac{-1}{PositionGap \cdot PositionLength}}$. &BigQuery\\

$PositionGap$ & Relative difference between $p_{mid}$ and $p_{mkt}$, computed as $\left|\frac{p_{mid}}{p_{mkt}}-1 \right|$. & BigQuery\\

$PositionLength$ & Price range length of a position, computed as $\frac{p_{upper}-p_{lower}}{p_{mid}}$. & BigQuery\\

$Return$ & 1min return of ETH/USD. & Binance\\

$Size$ & Hypothetical trade size in 100, 500, 1K, 5K, 10K, 50K, 100K, 500K, 1M (in \$). &\\

$Slippage$ & Slippage, computed as $\left|\frac{p_{avg}}{p_{mkt}}-1\right|$. Please refer to Section 4.1 for details on $p_{avg}$ computation on Uniswap v3. & BigQuery\\

$TVL$ & Total value locked, i.e. \$ value of all the liquidity in the pool. & BigQuery\\

$Volatility$ & Realized volatility of ETH/USD over the previous 24 hours, computed as the square root of the sum of squared 1min $Returns$ over previous 24 hours. & Binance\\

$Volume$ & Traded volume over previous 24 hours, computed every minute (in \$). & BigQuery\\\hline

\end{tabular}
